Spatially-resolved Stellar Population Properties of the M 51-NGC 5195 System from Multi-wavelength Photometric Data

Using multi-band photometric images of M 51 and its companion NGC 5195 from ultraviolet to optical and infrared, we investigate spatially resolved stellar population properties of this interacting system with stellar population synthesis models. The observed IRX is used to constrain dust extinction. Stellar mass is also inferred from the model fitting. By fitting observed spectral energy distributions (SEDs) with synthetical ones, we derive two-dimensional distributions of stellar age, metallicity, dust extinction, and stellar mass. In M 51, two grand-designed spiral arms extending from the bulge show young age, rich metallicity, and abundant dust. The inter-arm regions are filled with older, metal-poorer, and less dusty stellar populations. Except for the spiral arm extending from M 51 into NGC 5195, the stellar population properties of NGC 5195 are quite featureless. NGC 5195 is much older than M 51, and its core is very dusty with $A_V$ up to 1.67 mag and dense in stellar mass surface density. The close encounters might drive the dust in the spiral arm of M51 into the center of NGC 5195.

==> bib.1 <==
\begin{thebibliography}{99}
%% you can type \apj for ApJ, \aap for A&A, \apss for Ap&SS, etc. Please consult
%% the macro chjaa.cls. You can also find them in aasguide.tex (AASTeX for ApJ, AJ, PASP)
%% Please follow the format of ChJAA's reference list

%\bibitem[Asplund et al.(2009)]{asplund09} Asplund, M., Grevesse, N., Sauval, A.~J., et al.\ 2009, \araa, 47, 481
  \bibitem[Bertin(2010)]{bertin02} Bertin, E.\ 2010, SWarp: Resampling and Co-adding FITS Images Together, ascl:1010.068
  %\bibitem[Bertin et al.(2002)]{bertin02} Bertin E., Mellier Y., Radovich M., Missonnier G., Didelon P., Morin B. 2002, in Astronomical Data Analysis Software and Systems XI, ASP Conf. Series 281, 228

  \bibitem[Boselli et al.(2003)]{bos03} Boselli, A., Gavazzi, G., \& Sanvito, G.\ 2003, \aap, 402, 37
  
  \bibitem[Bresolin et al.(2004)]{bre04} Bresolin, F., Garnett, D.~R., \& Kennicutt, R.~C., Jr.\ 2004, \apj, 615, 228

  \bibitem[Bruzual A.~\& Charlot(1993)]{bru93} Bruzual A., G., \& Charlot, S.\ 1993, \apj, 405, 538

  \bibitem[Bruzual \& Charlot(2003)]{bru03} Bruzual, G., \& Charlot, S.\ 2003, \mnras, 344, 1000

  \bibitem[Bruzual(2007)]{bru07} Bruzual, A.~G.\ 2007, Stellar Populations as Building Blocks of Galaxies, 241, 125
  
  \bibitem[Burstein et al.(1994)]{bur94} Burstein, D., Hester, J.~J., Windhorst, R.~A., et al.\ 1994, Bulletin of the American Astronomical Society, 26, 41.10
  
  \bibitem[Calzetti et al.(2005)]{cal05} Calzetti, D., Kennicutt, R.~C., Jr., Bianchi, L., et al.\ 2005, \apj, 633, 871
  
  \bibitem[Cardelli et al.(1989)]{car89} Cardelli, J.~A., Clayton, G.~C., \& Mathis, J.~S.\ 1989, \apj, 345, 245
  
  \bibitem[Chabrier(2003)]{cha03} Chabrier, G.\ 2003, \pasp, 115, 763
  
  \bibitem[Chambers et al.(2016)]{cha16} Chambers, K.~C., Magnier, E.~A., Metcalfe, N., et al.\ 2016, arXiv:1612.05560
  
  \bibitem[Charlot \& Bruzual A(1991)]{cha91} Charlot, S., \& Bruzual A, G.\ 1991, \apj, 367, 126
  
  \bibitem[Cort{\'e}s et al.(2006)]{cor06} Cort{\'e}s, J.~R., Kenney, J.~D.~P., \& Hardy, E.\ 2006, \aj, 131, 747
  
  \bibitem[Croxall et al.(2015)]{croxall15} Croxall, K.~V., Pogge, R.~W., Berg, D.~A., et al.\ 2015, \apj, 808, 42.
  
  \bibitem[Dark Energy Survey Collaboration et al.(2016)]{des16} Dark Energy Survey Collaboration, Abbott, T., Abdalla, F.~B., et al.\ 2016, \mnras, 460, 1270
  
  \bibitem[De Looze et al.(2014)]{looze14} De Looze, I., Fritz, J., Baes, M., et al.\ 2014, \aap, 571, A69
  
  %\bibitem[Dey et al.(2018)]{dey18} Dey, A., Schlegel, D.~J., Lang, D., et al.\ 2018, arXiv:1804.08657
  \bibitem[Dey et al.(2019)]{dey18} Dey, A., Schlegel, D.~J., Lang, D., et al.\ 2019, \aj, 157, 168
  
  \bibitem[Dobbs et al.(2010)]{dob10} Dobbs, C.~L., Theis, C., Pringle, J.~E., \& Bate, M.~R.\ 2010, \mnras, 403, 625
  
  \bibitem[Eldridge \& Stanway(2009)]{eld09} Eldridge, J.~J., \& Stanway, E.~R.\ 2009, \mnras, 400, 1019
  
  \bibitem[Engelbracht et al.(2010)]{engelbracht10} Engelbracht, C.~W., Hunt, L.~K., Skibba, R.~A., et al.\ 2010, \aap, 518, L56

  
  \bibitem[Fan et al.(1996)]{fan96} Fan, X., Burstein, D., Chen, J.-S., et al.\ 1996, \aj, 112, 628
  
  \bibitem[Feldmeier et al.(1997)]{fel97} Feldmeier, J.~J., Ciardullo, R., \& Jacoby, G.~H.\ 1997, \apj, 479, 231
  
  \bibitem[Fioc \& Rocca-Volmerange(1997)]{fio97} Fioc, M., \& Rocca-Volmerange, B.\ 1997, \aap, 326, 950
  
  \bibitem[Fischera \& Dopita(2005)]{fis05} Fischera, J., \& Dopita, M.\ 2005, \apj, 619, 340
  
  \bibitem[Fisher \& Drory(2008)]{fis08} Fisher, D.~B., \& Drory, N.\ 2008, \aj, 136, 773
  
  \bibitem[Fisher \& Drory(2010)]{fis10} Fisher, D.~B., \& Drory, N.\ 2010, \apj, 716, 942
  
  \bibitem[Fisher et al.(2009)]{fisher09} Fisher, D.~B., Drory, N., \& Fabricius, M.~H.\ 2009, \apj, 697, 630
  
  \bibitem[Gaia Collaboration et al.(2016)]{gai16} Gaia Collaboration, Brown, A.~G.~A., Vallenari, A., et al.\ 2016a, \aap, 595, A2
  
  \bibitem[Gallazzi, \& Bell(2009)]{gallazzi09} Gallazzi, A., \& Bell, E.~F.\ 2009, \apjs, 185, 253
  
  \bibitem[Goad et al.(1979)]{goad79} Goad, J.~W., de Veny, J.~B., \& Goad, L.~E.\ 1979, \apjs, 39, 439
  
  \bibitem[Grillmair et al.(1997)]{grillmair97} Grillmair, C.~J., Faber, S.~M., Lauer, T.~R., et al.\ 1997, \aj, 113, 225
  
  \bibitem[Hao et al.(2011)]{hao11} Hao, C.-N., Kennicutt, R.~C., Johnson, B.~D., et al.\ 2011, \apj, 741, 124
  
  \bibitem[Ho et al.(2009)]{ho09} Ho, L.~C., Greene, J.~E., Filippenko, A.~V., \& Sargent, W.~L.~W.\ 2009, \apjs, 183, 1
  
  \bibitem[Jarrett et al.(2003)]{jarrett03} Jarrett, T.~H., Chester, T., Cutri, R., Schneider, S.~E., \& Huchra, J.~P.\ 2003, \aj, 125, 525
  
  \bibitem[Kaleida \& Scowen(2010)]{Kaleida2010} Kaleida, C., \& Scowen, P.~A.\ 2010, \aj, 140, 379
  
  \bibitem[Kennicutt et al.(2003)]{kennicutt03} Kennicutt, R.~C., Jr., Bresolin, F., \& Garnett, D.~R.\ 2003, \apj, 591, 801
  
  \bibitem[Kewley et al.(2006)]{kewley06} Kewley, L.~J., Geller, M.~J., \& Barton, E.~J.\ 2006, \aj, 131, 2004
  
  \bibitem[Kohno et al.(2002)]{kohno02} Kohno, K., Tosaki, T., Matsushita, S., et al.\ 2002, \pasj, 54, 541

  
  \bibitem[Kong et al.(2000)]{kong00} Kong, X., Zhou, X., Chen, J., et al.\ 2000, \aj, 119, 2745
  
  \bibitem[Kotulla et al.(2009)]{kotulla09} Kotulla, R., Fritze, U., Weilbacher, P., \& Anders, P.\ 2009, \mnras, 396, 462
  
  \bibitem[Kormendy \& Kennicutt(2004)]{Kormendy04} Kormendy, J., \& Kennicutt, R.~C., Jr.\ 2004, \araa, 42, 603
  
  \bibitem[Kormendy et al.(2010)]{Kormendy10} Kormendy, J., Drory, N., Bender, R., \& Cornell, M.~E.\ 2010, \apj, 723, 54
  
  %\bibitem[Kroupa(2001)]{kroupa01} Kroupa, P.\ 2001, \mnras, 322, 231
  
  \bibitem[Kuntz et al.(2008)]{kuntz08} Kuntz, K.~D., Harrus, I., McGlynn, T.~A., Mushotzky, R.~F., \& Snowden, S.~L.\ 2008, \pasp, 120, 740
  
  \bibitem[Li et al.(2004a)]{li04a} Li, J., Ma, J., Zhou, X., et al.\ 2004a, \aap, 420, 89
  
  \bibitem[Li et al.(2004b)]{li04b} Li, J.-L., Zhou, X., Ma, J., \& Chen, J.-S.\ 2004b, \cjaa, 4, 143
  
  \bibitem[Lin et al.(2013)]{lin13} Lin, L., Zou, H., Kong, X., et al.\ 2013, \apj, 769, 127
  
  \bibitem[Lamers et al.(2002)]{lamers02} Lamers, H.~J.~G.~L.~M., Panagia, N., Scuderi, S., et al.\ 2002, \apj, 566, 818
  
  \bibitem[Leitherer et al.(1999)]{leitherer99} Leitherer, C., Schaerer, D., Goldader, J.~D., et al.\ 1999, \apjs, 123, 3
  
  \bibitem[Maraston(2005)]{maraston05} Maraston, C.\ 2005, \mnras, 362, 799
  
  \bibitem[Martin et al.(2005)]{martin05} Martin, D.~C., Fanson, J., Schiminovich, D., et al.\ 2005, \apjl, 619, L1
  
  \bibitem[Mason et al.(2001)]{mas01} Mason, K.~O., Breeveld, A., Much, R., et al.\ 2001, \aap, 365, L36
  
  \bibitem[Martig et al.(2009)]{martig09} Martig, M., Bournaud, F., Teyssier, R., et al.\ 2009, \apj, 707, 250
  
  \bibitem[Men{\'e}ndez-Delmestre et al.(2007)]{menendez-delemestre07} Men{\'e}ndez-Delmestre, K., Sheth, K., Schinnerer, E., Jarrett, T.~H., \& Scoville, N.~Z.\ 2007, \apj, 657, 790
  
  \bibitem[Mentuch Cooper et al.(2012)]{men12} Mentuch Cooper, E., Wilson, C.~D., Foyle, K., et al.\ 2012, \apj, 755, 165
  
  \bibitem[Meurer et al.(1999)]{meurer99} Meurer, G.~R., Heckman, T.~M., \& Calzetti, D.\ 1999, \apj, 521, 64
  
  \bibitem[Morrissey et al.(2007)]{morrissey07} Morrissey, P., Conrow, T., Barlow, T.~A., et al.\ 2007, \apjs, 173, 682
  
  \bibitem[Moustakas et al.(2010)]{moustakas10} Moustakas, J., Kennicutt, R.~C., Jr., Tremonti, C.~A., et al.\ 2010, \apjs, 190, 233
  
  \bibitem[Mu{\~n}oz-Mateos et al.(2009)]{munoz09} Mu{\~n}oz-Mateos, J.~C., Gil de Paz, A., Boissier, S., et al.\ 2009, \apj, 701, 1965
  
  \bibitem[Nikola et al.(2001)]{nikola01} Nikola, T., Geis, N., Herrmann, F., et al.\ 2001, \apj, 561, 203
  
  \bibitem[Oke \& Gunn(1983)]{oke83} Oke, J.~B., \& Gunn, J.~E.\ 1983, \apj, 266, 713
  
  \bibitem[Ro{\v s}kar et al.(2008)]{roskar08} Ro{\v s}kar, R., Debattista, V.~P., Stinson, G.~S., et al.\ 2008, \apjl, 675, L65
  
  \bibitem[Salo \& Laurikainen(2000)]{salo00} Salo, H., \& Laurikainen, E.\ 2000, \mnras, 319, 393
  
  \bibitem[Schlegel et al.(1998)]{schlegel98} Schlegel, D.~J., Finkbeiner, D.~P., \& Davis, M.\ 1998, \apj, 500, 525
  
  \bibitem[Silva et al.(2016)]{silva16} Silva, D. J., Blum, R. D., Allen, L., et al.\ 2016, in AAS Meeting \#228, 317.02
  
  \bibitem[Skrutskie et al.(2006)]{skrutskie06} Skrutskie, M.~F., Cutri, R.~M., Stiening, R., et al.\ 2006, \aj, 131, 1163
  
  \bibitem[Spillar et al.(1992)]{spillar92} Spillar, E.~J., Oh, S.~P., Johnson, P.~E., \& Wenz, M.\ 1992, \aj, 103, 793
  
  \bibitem[Toomre \& Toomre(1972)]{toomre72} Toomre, A., \& Toomre, J.\ 1972, \apj, 178, 623
  
  \bibitem[Tully(1974)]{tully74} Tully, R.~B.\ 1974, \apjs, 27, 449
  
  \bibitem[Walter et al.(2008)]{walter08} Walter, F., Brinks, E., de Blok, W.~J.~G., et al.\ 2008, \aj, 136, 2563
  
  \bibitem[Werner et al.(2004)]{Werner04} Werner, M.~W., Roellig, T.~L., Low, F.~J., et al.\ 2004, \apjs, 154, 1
  
  \bibitem[White \& Rees(1978)]{white78} White, S.~D.~M., \& Rees, M.~J.\ 1978, \mnras, 183, 341
  
  \bibitem[Williams et al.(2009)]{williams09} Williams, B.~F., Dalcanton, J.~J., Dolphin, A.~E., Holtzman, J., \& Sarajedini, A.\ 2009, \apjl, 695, L15
  
  \bibitem[York et al.(2000)]{york00} York, D.~G., Adelman, J., Anderson, J.~E., Jr., et al.\ 2000, \aj, 120, 1579
  
  \bibitem[Zacharias et al.(2010)]{zacharias10} Zacharias, N., Finch, C., Girard, T., et al.\ 2010, \aj, 139, 2184
  
  \bibitem[Zaritsky et al.(1994)]{zaritshy94} Zaritsky, D., Kennicutt, R.~C., Jr., \& Huchra, J.~P.\ 1994, \apj, 420, 87
  
  \bibitem[Zhou et al.(2001)]{zhou01} Zhou, X., Jiang, Z.-J., Xue, S.-J., et al.\ 2001, \cjaa, 1, 372
  
  \bibitem[Zibetti et al.(2009)]{zibetti09} Zibetti, S., Charlot, S., \& Rix, H.-W.\ 2009, \mnras, 400, 1181.
  
  \bibitem[Zou et al.(2011)]{zou2011} Zou, H., Zhang, W., Yang, Y., et al.\ 2011, \aj, 142, 16
  
  \bibitem[Zou et al.(2017a)]{zou2017} Zou, H., Zhou, X., Fan, X., et al.\ 2017a, \pasp, 129, 064101
  
  \bibitem[Zou et al.(2017b)]{zou2017aj} Zou, H., Zhang, T., Zhou, Z., et al.\ 2017b, \aj, 153, 276
  
  \bibitem[Zou et al.(2018)]{zou18} Zou, H., Zhang, T., Zhou, Z., et al.\ 2018, \apjs, 237, 37

\end{thebibliography}

